Stable Matching: Choosing Which Proposals to Make

To guarantee all agents are matched in general, the classic Deferred Acceptance algorithm needs complete preference lists. In practice, preference lists are short, yet stable matching still works well. This raises two questions: $\bullet$ Why does it work well? $\bullet$ Which proposals should agents include in their preference lists? We study these questions in a model, introduced by Lee [17], with preferences based on correlated cardinal utilities: these utilities are based on common public ratings of each agent together with individual private adjustments. Lee showed that for suitable utility functions, in large markets, with high probability, for most agents, all stable matchings yield similar valued utilities. By means of a new analysis, we strengthen Lee's result, showing that in large markets, with high probability, for $\it all$ but the agents with the lowest public ratings, all stable matchings yield similar valued utilities. We can then deduce that for $\it all$ but the agents with the lowest public ratings, each agent has an easily identified length $O(\log n)$ preference list that includes all of its stable matches, addressing the second question above. We note that this identification uses an initial communication phase. We extend these results to settings where the two sides have unequal numbers of agents, to many-to-one settings, e.g. employers and workers, and we also show the existence of an $\epsilon$-Bayes-Nash equilibrium in which every agent makes relatively few proposals. These results all rely on a new technique for sidestepping the conditioning between the tentative matching events that occur over the course of a run of the Deferred Acceptance algorithm. We complement these theoretical results with an experimental study.

==> conclusion.tex <==
\section{Discussion and Open Problems}
\label{sec:discussion}

Our work shows that in the bounded derivatives model, apart from a sub-constant fraction of the
agents, each of the other agents has $O(\ln n)$ easily identified edges on their preference list which cover all
their stable matches w.h.p. 

As we will see in Section~\ref{sec:simulations},
our experiments for the one-to-one setting yield a need for what appear to be impractically large preference lists. 
While the results in the many-to-one setting are more promising, even here
the preference lists appear to be on the large side.
Also, while our rule for identifying the edges to include is simple,
in practice it may well require too much communication to identify these edges.
At the same time, our outcome is better than what is achieved in practice: we obtain a complete match
with high probability, whereas in the NRMP setting a small but significant percentage of positions are left unfilled.
Our conclusion is that it remains important to understand how to effectively select smaller sets of edges.

In the popularity model, it is reasonable for each agent to simply select their favorite partners. But in the current setting, which we consider to be more realistic, it would be an ineffective strategy, as it would result in most agents remaining unmatched.
%
Consequently, we believe the main open issue is to characterize what happens when the number of edges $k$ that an agent can list
is smaller than the size of the allowable edge set.
We conjecture that following a simple protocol for selecting edges to list, such as the one
we use in our experiments (see Section \ref{sec:const-no-props}), will lead to an $\eps$-Bayes-Nash equilibrium, where $\eps$ is a decreasing function of $k$. Strictly speaking, as the identification of allowable edges requires communication,
we need to consider the possibility of strategic communication,
and so one would need to define a notion of $\eps$-equilibrium akin to a Subgame Perfect equilibrium.
We conjecture that even with this, it would still be an $\eps$-equilibrium.

Finally, it would be interesting to resolve whether the experimentally observed near uniqueness of the stable match
for non-bottom agents is a property of the linear separable model.
We conjecture that in fact it also holds in the bounded derivatives model.
% Perhaps it holds even in the general values model, but this is less clear to us.




==> eps-nash-const-props.tex <==

\section{$\eps$-Nash equilibrium with expected $O(1)$ proposals per agent}
\label{sec::equil-Oh-one-props}

We consider the following set-up in which all but the bottommost agents
each make $k$ proposals in expectation, and the bottommost agents each make up to $O(k^2)$ proposals
in expectation.
We define $\sigma = \tfrac 12(k/n)^{1/3}$.

There will be two communication rounds in which the eventual proposals are identified.
First, each woman $w$ with public rating $r_w$ will request interviews with some of the men whose public rating 
is in the cone $r_w\pm \sigma$: the men receiving requests are those
for whom she has a private score which is at least as large as a cutoff that depends on her public rating.
The men accept the interview requests from the women for whom they have a private score, which again
is at least as large as a cutoff that depends on their public rating.

If the woman's public rating lies in the range $[\sigma,1-\sigma]$, then the cutoff is
$1-2\sigma$, and similarly for the men. We define the cutoffs for the remainder of the public rating range later.

We note that this definition of the communication rounds is not identical to the previous setup when $k=\Theta(\ln n)$.
However, we chose to modify the setup here in order to simplify the analysis.


For women with public rating in the range $[\sigma,1-\sigma]$,
the expected number of men in the cone is $2\sigma=(k/n)^{1/3}\cdot n$, so the expected
number of interviews granted to a woman is $(2\sigma)^3 \cdot n = k$. 
For women and men with public rating in the range $[1-\sigma,1]$ we adjust the cutoffs so that
the expected number of interviews granted remains at $k$.
For the agents with public rating in the range $[0,\sigma]$ we adjust the cutoffs, allowing the
number of interviews granted to grow to $\Theta(k^2)$.

The pairs for which interviews are granted are the proposals that are submitted to the DA algorithm.
We call these edges the Selected Edge Set.

We note that in reality, private scores are fully determined by the interviews.
However, as these are the only private scores that are fully determined,
it seems reasonable to treat the other private scores as being smaller,
as the eventual match would be the same if they were smaller.
\RJC{Not sure we want to say this.}



Our goal, for all men $m$ and women $w$, is to have edge $(m,w)$ be in the Selected Edge Set with probability $p_{s_m,s_w}$, where $p_{s_m,s_w}=p_{s_w,s_m}$ and
$\int_{s_m-\sigma}^{s_m+\sigma} p_{s_w,r} \text{d}r=k$ (and therefore
$\int_{s_w-\sigma}^{s_w+\sigma} p_{r,s_m} \text{d}r=k$ also); we define $p_{xy}=0$ if $|x-y|>2\sigma$, $x>1$, $y>1$, $x<0$, or $x>1$.
We provide a solution below.

\begin{lemma}
There is a choice of values $p_{xy}$, such
that for $|x-y|, |x-z|\le 2\sigma$, and $0\le x,y,z\le 1$, $\max\{p_{xy}/ p_{xz}\} \le 3$ (and therefore
$\max\{p_{xz}/p_{yz}\} \le 3$ also).
\end{lemma}
\begin{proof}
This can be achieved by
setting $p_{xy}= k/4\sigma^2$ if $x$ or $y\in[\sigma,1-\sigma]$,
$p_{xy}= k/4\sigma^2+k(\sigma-x)(\sigma-y)/2\sigma^2$ if both $x,y< \sigma$, and
$p_{xy}= k/4\sigma^2+k(x+\sigma-1)(y+\sigma-1)/2\sigma^2$ if both $x,y> 1-\sigma$.
\end{proof}

Each woman $w$ requests interviews from man $m$ in $M[s_w-\sigma,s_w+\sigma]$ if $w$'s private score for $m$, $v_w(m) \ge (p_{s_d,s_h})^{1/2}$;
similarly, a man will accept a request
only if its private score $v_m(w) \ge (p_{s_d,s_h})^{1/2}$.
Clearly, edge $(m,w)$ is selected with probability $p_{s_d,s_h}$.

Later, we will change the probabilities when at least one of $x,y<\sigma$.

\smallskip

Our analysis of DA will ignore the communication protocol.
Instead, the women will propose in the usual order of preference, those edges for which she would request interviews.
The men will only consider those proposals which correspond to interview requests that they would accept.
We see that in this run of DA the edges that form tentative matches are all in the Interview Edge Set,
and therefore we get the same outcome as we would if running DA on the Interview Edge Set.
Henceforth, we refer to the edges the women propose as proposals (remembering that these correspond to interview requests).

We begin by restating and reproving Lemma~\ref{lem::key_bounded} to account for the new set up including the
the fact that some agents will fail to match.

We will need to parameterize the new bound by the difference in the number of non-matches on the two sides, as follows.

\begin{defn}
\label{def::failure-diff}
Fix $i$. Let $w_i$ be the rank $i$ woman and $r_i$ be her public rating.
Suppose we run woman proposing DA only using edges for which the man has value at least $U(r_i,1)$ and for
which the woman has value at least $V(r_i,1)$.
We call this the \emph{restricted edge set}.
Among the women with public rating at least $r_i+\sigma$, let $F_W$ denote the subset of women who fail to match and let $f_w= |F_W|/n$. 
Similarly, among the men with public rating at least $r_i+\sigma$, let $F_M$ denote the subset of women who fail to match and let $f_m= |F_M|/n$.
We define the \emph{failure difference}, $f_d=f_w-f_m$. Strictly, this notation should be parameterized by $i$; 
for the sake of readability, we suppress this index for now.
\end{defn}
\begin{claim}
\label{clm::f-equals-final-value}
Consider a run of woman-proposing DA on the full set of edges.
Then among the women with public rating at least $r_i+\sigma$, the women who fail to match are exactly the women in $F_W$,
and among the men with public rating at least $r_i+\sigma$, the men who fail to match are exactly the women in $F_M$.
If, instead, we run man-proposing DA on the full set of edges, the same sets of men and women fail to match.
\end{claim}
\begin{proof}
We first note that when using the full set of edges, whether we run woman-proposing DA or man-proposing DA,
the same men and women will remain unmatched (this follows from the fact that woman-proposing DA is woman-optimal and man-pessimal,
and man-proposing DA is man-optimal and woman-pessimal, and the observation that in each run the numbers of unmatched men and women are equal).

The observation also applies to the runs of woman-proposing and man-proposing DA when limited to the restricted edge set.

Consider a run of woman-proposing DA only using the restricted edge set.
Suppose woman $w$ with public rating $r_w \ge r_i+\sigma$ remains unmatched.
Necessarily, she will be unmatched in the run of woman-proposing DA using the full edge set, as a woman's match only gets worse as more edges are proposed.

Now suppose $w$ is matched in the run of woman-proposing DA only using the restricted edge set.
Then, by the second observation, $w$ is also matched in the the run of man-proposing DA on the restricted edge set.
Necessarily, she will be matched in the run of man-proposing DA using the full edge set, as her match only improves as more edges are proposed.
By the first observation, she will also be matched in the run of woman-proposing DA using the full edge set.

This shows that among the women with public rating at least $r_i+\sigma$, the women who fail to match are exactly the women in $F_W$.
The claim regarding $F_M$ follows analogously.
\end{proof}

\begin{lemma}\label{lem::key_bounded_var}
Let $m_i$ be a man with public rating $r_{m_i}\ge \sigma$.
Let $\alpha=\tfrac13\sigma$, let $L>0$ be given, and suppose that $\beta$ and $\gamma$ satisfy
\eqref{eqn::beta-constraint} and \eqref{eqn::gamma-constraint}, respectively.
Suppose also that 
woman-proposing DA is run with double cut at the rank $i$ man $m_{i}$ 
and public rating $r_{m_i} - \alpha$. 
Let $h_i=\big|M[r_{m_i} - \alpha,r_{m_i}]\setminus\{m_{i}\}\big|$ and
$\ell_i = h_i + \alpha n -1$.
Let $\overline{w}_i$ be the woman with rank $i+\ell_i$.
Then, the following event occurs with probability at least $1-p_f$,
where the failure probability 
$p_f=n\cdot \exp(-\alpha(n-1)/12)
+n\cdot \exp(-\alpha n/24)
    +2n^{-(c+1)}
    +n \exp(-\alpha n \exp(-\alpha\beta\gamma n)/24)$:

Among the men $m_i$ such that $r_{m_i}\ge \sigma$, $\overline{w}_i$ exists,
and for all but
$\alpha n \cdot\exp(-\frac 14\alpha\beta\gamma n)$ of these men,
between them the $i+\ell_i$ women in $W[r_{\overline{w}_i},1]$ make at least one proposal that is accepted by $m_{i}$. 
\end{lemma}


The first change in the analysis is to the statement and proof of Claim~\ref{clm::many-man-acceptable-props}.
The new version of the lemma follows.

\begin{claim}
\label{clm::many-man-acceptable-props-const-props}
Suppose that $f_d\ge -\tfrac 12 \alpha$.
Let ${\mathcal B}_3$ be the event that between them, the women with
rank at most $i+\ell_i$ make fewer than
$\tfrac 12 (\alpha+f_d)\beta n$ Step 2 proposals to $m_i$.
If events ${\mathcal B}_1$ and ${\mathcal B}_2$
do not occur, then ${\mathcal B}_3$ occurs with probability at most $\exp(-(\alpha+f_d)\beta n/8)$.
The only randomness used in the proof are the choices of the  women's private scores.
\end{claim}
\begin{proof}
Previously, we observed that:
At each leaf of $T$, up to 
$i+h_i -1= i+\ell_i - \alpha n$
women will have been matched with someone other than $m_i$.
Now, we argue as follows.
At the end of the double cut run, excluding $m_i$, at most $i +h_i-1 -f_m\cdot n$ men are matched, i.e.\ have accepted a proposal;
this is because there are $i+h_i-1$ men at hand, and at the end of the full run of DA among the first $i-1$ men,
$f_m\cdot n$ will have refused all proposals, so at this time at least $f_m\cdot n$ will have refused all the proposals they have received.
There are $i+\ell_i =i+h_i -1 +\alpha n$ women making proposals.
Among the first $i-1$ women, of the $f_w\cdot n$ who will run through all their proposals in the full run of DA,
at the end of Step 1 of the double cut run, at most $f_w\cdot n$ have done so.
This leaves at least $(i+\ell_i -f_w\cdot n) - (i +h_i-1 -f_m\cdot n)=\alpha n + (f_m-f_w)n=\alpha n +f_d\cdot n$ 
women who 
\begin{itemize}
    \item could make a proposal to $m_i$ (because $m_i$ lies
in their cone of potential requests), and
\item end Step 1 with no proposal accepted.
\end{itemize}

$(\alpha +f_d)n$ will replace the $\alpha n$ in the previous analysis.

What is the effect on the execution tree of conditioning on $f_w$ and $f_m$?
It may alter the probabilities of each path in the tree.
However, the analysis did not depend on the values of these probabilities,
so the argument is unaffected.
\end{proof}

In order to bound the number of mismatches w.h.p., we partition the men and women into 
consecutive mismatch intervals of $\alpha n$ men and $\alpha n$ women (i.e.\ the first $\alpha n$ men
and the first $\alpha n$ women, etc.).

We define $f_i$ to be the value of $f_d$ for $m_i$ and $w_i$.
Clearly, for all $i$, $|f_{i+1}-f(i)|n \le 1$.

\begin{lemma}
\label{lem::few-mismatches}
Suppose that events ${\cal B}_1$ and ${\cal B}_2$ do not occur.
Then, with failure probability at most $2n^{-(c+1)}$,
for all the mismatch intervals $I$, the following events, which we call ${\cal B}'_3$, occur. \\
\emph{Case 1}. For every $m_i \in I$, $f_i\ge 0$. \\
Then the number
of men in $I$ who fail to receive $\tfrac12\alpha\beta n$ proposals
is at most $\tfrac12\alpha n \cdot\exp(-\alpha\beta n/8) 
+ ((c+2)\tfrac12\alpha n \cdot \exp(-\alpha\beta n/8))^{1/2}$.\\
\emph{Case 2}. For every $m_i \in I$, $f_i\le 0$. \\
Then the number
of women in $I$ who fail to fail to receive $\tfrac12\alpha\beta n$ proposals is at most 
$\tfrac12\alpha n \cdot\exp(-\alpha\beta n/8) 
+ ((c+2)\tfrac12\alpha n \cdot \exp(-\alpha\beta n/8))^{1/2}$.\\
\emph{Case 3}. For every $m_i \in I$, $-\alpha n/2\le f_i \le \alpha n/2$.\\
Then the number of men in $I$ who fail to fail to receive $\tfrac14\alpha \beta$ proposals is at most 
$\tfrac14\alpha n \cdot \exp(-\alpha\beta n/16) 
+ ((c+2)\tfrac 14\alpha n \cdot \exp(-\alpha\beta n/16))^{1/2}$
as is the number of women.

For large enough $n$, these bounds on the number of agents in $I$ are all 0.
\end{lemma}
\begin{proof}
Case 1. By Claim~\ref{clm::many-man-acceptable-props-const-props},
each man $m_i$ fails to receive $\tfrac 12\alpha \beta n$ proposals with probability at most $\exp(-\alpha\beta n/8)$.
Furthermore, these events depend on the women's private scores for $m_i$ and hence are independent.
The expected number of men not receiving $\tfrac 12 \alpha \beta n$ proposals is at most
$\tfrac 12 \alpha n \cdot \exp(-\alpha\beta n/8)$.
By a Chernoff bound, the bound is at most
$\tfrac 12 \alpha n \cdot \exp(-\alpha\beta n/8) + [(c+2)\tfrac 12 \alpha n \cdot \exp(-\alpha\beta n/8)]^{1/2}$
with failure probability at most $n^{-(c+2)}$.

The analysis of Case 2 is symmetric.

Case 3. By Claim~\ref{clm::many-man-acceptable-props-const-props},
each man $m_i$ fails to receive $\tfrac 12(\alpha-\tfrac 12\alpha) \beta n = \tfrac 14 \alpha \beta n$ proposals with probability at most $\exp(-\tfrac 12\alpha\beta n/8)=\exp(-\alpha\beta n/16)$.
The expected number of men not receiving $\tfrac 14 \alpha \beta n$ proposals is at most
$\tfrac 14 \alpha n \exp(-\alpha\beta n/16)$.
By a Chernoff bound, the bound is at most
$\tfrac 14 \alpha n \exp(-\alpha\beta n/16) + [(c+2)\tfrac 14 \alpha n \exp(-\alpha\beta n/16)]^{1/2}$
with failure probability at most $n^{-(c+2)}$.
The same bound applies to the women.

Each sequence $s$ of possible interval types (obeying Cases 1--3, respectively) occurs with some probability $p_s$.
The overall failure probability is the sum of the failure probabilities over the possible sequences.
But the failure probability for sequence $s$ needs to be multiplied by $p_s$.
Thus the overall failure probability is at most $2n \cdot n^{-(c+2)} \le 2 n^{-(c+1)}$.

For large enough $n$, as the numbers of men and women are integral, 
the bounds on the numbers of men and women are less than one and hence zero with failure probability at most $2 n^{-c(+1)}$.
\end{proof}

\begin{cor}
\label{cor::joint-mismatch-bound}
Suppose none of ${\cal B}_1$, ${\cal B}_2$ and ${\cal B}'_3$ occur.
Then the number of unmatched men in the first $h$ intervals is at most
$h\alpha n \exp(-\frac 14\alpha\beta\gamma n)$
with failure probability
at most $n \exp(-\alpha n \exp(-\frac 14\alpha\beta\gamma n)/6)$.
\end{cor}
\begin{proof}
We prove the bound by induction on $h$.

Suppose man $m_i$ receives at least $\tfrac 14 \alpha \beta n$ proposals.
The probability that $m_i$ accepts none of them is at most
$(1 - \gamma)^{\tfrac 14 \alpha \beta n} \le \exp(-\frac14\alpha\beta\gamma n)$.
Thus in Cases 1 and 3, the expected number of men in the $h$-th interval who do not match is at most
$\tfrac 12\alpha n \cdot \exp(-\frac 14\alpha\beta\gamma n)$, and as the outcome for $m_i$ is
based on his private scores, these events are independent.
Therefore, by a Chernoff bound, the number of men not matching is at most
$\alpha n \cdot\exp(-\frac 14\alpha\beta\gamma n)$ with failure probability
at most $\exp(-\alpha n \exp(-\frac 14\alpha\beta\gamma n)/6)$.

Whenever $f_i\ge 0$, the number of unmatched men, up to but not including $m_i$ is at least
the number of mismatched women. Thus in Case 1, the bound will apply to the men in the $h$-th
interval by the argument in the preceding paragraph, and therefore also to the women.
The same argument applies for Case 2.
In Case 3, the bounds apply directly to both the men and women.
\end{proof}




==> linear.tex <==
\section{Upper Bound in The Linear Separable Model}
\label{sec::linear}

To illustrate our proof technique for deriving upper bounds, we begin by stating and proving our upper bound result for the special case of the linear separable model with $\lambda= \tfrac 12$. 

\begin{theorem}\label{thm::basic-linear-result}
In the linear separable model with $\lambda=1/2$, when there are $n$ men and $n$ women,
for any given constant $c>0$, for large enough $n$, with probability at least $1-n^{-c}$, in every stable match, for every $i$, if $r_{w_i}\ge \sigmabar\triangleq 3\Lbar/2$, 
agent $m_i$ suffers a loss of at most $\Lbar$, where $\Lbar=(16(c+2)\ln n/n)^{1/3}$,
and similarly for the agents $w_i$.
\end{theorem}
Note that w.h.p., the public scores of aligned agents are similar.

In words, w.h.p., all but the bottommost agents (those whose aligned agents have %has 
public rating less than $\sigmabar$) suffer a loss of no more than $\Lbar$. We call this high probability outcome $\mathcal E$.

This is a special case of our basic upper bound for the bounded utilities model (Theorem \ref{thm:basic-bdd-deriv-result}).\\

One of our goals is to be able to limit the number of proposals the proposing side needs to make.
We identify the edges that could be in some stable matching assuming $\mathcal E$ occurs, calling them acceptable edges.
Our definition is stated generally so that it covers all our results.

\begin{defn} [Acceptable edges] 
Let $0<\sigma <1$ and $0<L<1$ be two parameters.
An edge $(m_i,w_j)$
is $(L,\sigma)$-\emph{man-acceptable} \rjc{either} if it provides $m_i$ utility at least $U(r_{w_i},1)-L$, or if $m_i\in M[0,\sigma)$.
The definition of $(L,\sigma)$-woman-acceptable is symmetric. $(m_i,w_j)$ is $(L,\sigma)$-\emph{acceptable} if it is both $(L,\sigma)$-man and $(L,\sigma)$-woman-acceptable.
\end{defn}

To prove our various results, we choose $L$ and $\sigma$ so that w.h.p.\ the edges in every stable matching are $(L,\sigma)$-\emph{acceptable}.
Again, we call this high probability event $\mathcal E$.
We will show that if $\mathcal E$ occurs, then running DA on the set of acceptable edges, or any superset of the acceptable edges
obtained via loss thresholds, 
produces the same stable matching as running DA on the full set of edges.

\begin{theorem}\label{lem::acceptable-suffice}
If E occurs, then running woman-proposing DA with the edge set restricted to the acceptable edges or to any superset of the acceptable edges obtained via loss thresholds (including the full edge set) result in the same stable matching.


\end{theorem}
The implication is that w.h.p.\ a woman can safely restrict her proposals to her acceptable edges, or to any overestimate of this set of edges obtained by her setting an upper bound on the loss she is willing to accept.
There is a small probability--- at most $n^{-c}$---that this may result in a less good outcome, which can happen only if
% namely the probability that 
$\mathcal E$ does not occur.
Note that Theorem~\ref{lem::acceptable-suffice} applies to every model we consider.
Then,
w.h.p., every stable matching gives each woman $w$, whose aligned agent $m$ has public rating $r_m\ge\sigmabar=\Omega((\ln n/n)^{1/3})$, a partner with public rating in the range $[r_m - 2\Lbar, r_m+\tfrac 52 \Lbar]$ (see appendix \ref{sec::cone-size}).
The bound $r_m-2\Lbar$ is a consequence of the bound on the woman's loss; the bound $r_m+\tfrac52\Lbar$ is a consequence of the bound on the men's losses. 
An analogous statement applies to the men. 

This means that if we are running woman-proposing DA, each of these women might as well limit her proposals to her woman-acceptable edges, which is at most the men with public ratings in the range $r_m \pm \Theta(\Lbar)$ for whom she has private scores of at least $1 - \Theta(\Lbar)$. (The constant in the second $\Theta$ term is the upper bound on the rate of change of $V$ w.r.t.\ the private score.) %value.)
In expectation, this yields $\Theta(n^{1/3}(\ln n)^{2/3})$ men to whom it might be worth proposing.
It also implies that a woman can have a gain of at most $\Theta(\Lbar)$ compared to her target utility.

If, in addition, each man can inexpensively signal the women who are man-acceptable to him,
either by means of a precise calculation, or by having an overestimate of his private scores, then the women can further limit their proposals to just those men providing them with a signal; in the case of accurate signals, this reduces the expected number of proposals these women can usefully make to just $\Theta(\ln n)$. 

\section{Sketch of the Proof of Theorem~\ref{thm::basic-linear-result}}
\label{sec::sketch-linear-result}

\rjc{
We now outline the main ideas used in our analysis (See Fig.~\ref{fig::key_bounded}.). 
We will analyze the outcome for each man $m_i$ separately, aside from those $m_i$ among the bottommost men.
Our goal is to show that w.h.p.\ each such $m_i$ receives $\Omega(\ln n/L)$ proposals, for then
w.h.p.\ one of these proposals provides $m_i$ a loss of at most $L$.
To this end, we identify a set $M_i$ of men which includes $m_i$ and a somewhat larger set $\widetilde{W}_i$ of women, both
defined in terms of a minimum public rating.
We then focus of an initial portion of a run of woman-proposing DA in which the proposals are limited
to being from women in $\widetilde{W}_i$ to men in $M_i$.
The key observation is that at  least $\big|\widetilde{W}_i\big| - \big|M_i\big|$ of these
women will end up unmatched, and therefore they
will run through all their available proposals.
By setting the parameters suitably, we are able to show that w.h.p.\ the proposals by the unmatched
women include $\Omega(\ln n/L)$ proposals to $m_i$.

To obtain this high probability bound we would
like to apply a Chernoff bound, which requires the various proposals to be independent.
Unfortunately, in general, this does not appear to be the case.
However, we are able to show that the failure probability for our setting is at most
the failure probability in an artificial setting in which the events are independent,
which yields the desired bound.
}

\begin{figure}[hbt]
\begin{center}
\begin{tikzpicture}
\begin{scope}[>=latex]
\draw (-0.2,3) to (-0.2,1.55);
\node at (-0.2,1.485) {$\circ$};
\node at (-2.8,1.485) {rating $r_{m_i}$, man $m_i$};
\draw[->] (-1.15,1.485) to (-0.45,1.485);
\node at (3,1.485) {$\circ$};
\node at (4.1,1.485) {woman $w_i$};
\draw[dashed] (0.2,1.485) to (2.9,1.485);
\draw (-0.2,1.46) to (-0.2,0.5);
\draw[<->] (-0.0,3) to (-0.0,0.5);
\node at (1.5,2.0) {$M_i=[r_{m_i}-\alpha,1]$};
\draw[<->] (-0.4,1.475) to (-0.4,0.5);
\node at (-2.5,1.0) {$h_i$ men, rating range $\alpha$};
\draw (3,3) to (3,1.55);
\draw (3,1.46) to (3,-0.95);
%\draw (3,-1) to (3,3);
\draw[<->] (3.2,1.475) to (3.2,-1);
\node at (4.1,0.25) {$\ell_i$ women};
\node at (0, 3.3) {men};
\node at (3, 3.3) {women};
\node at (-3.2,0.5) {cutoff $r_{m_i} - \alpha$};
\draw[->] (-1.9,0.5) to (-0.45,0.5);
\draw[<->] (5.0,3) to (5.0,-1);
\node at (6.4,1.0) {$\widetilde{W}_i=W[r_{\overline{w}_i},1]$};
\node at (3,-1) {$\circ$};
\node at (3.2,-1.3) {woman $\overline{w}_i=w_{i+\ell_i}$};
\end{scope}
\end{tikzpicture}
\end{center}
\caption{Illustrating Lemma~\ref{lem::key_bounded}} 
\label{fig::key_bounded}
%
\end{figure}


% Before entering into our analysis we introduce 
\rjc{We formalize the men's rating cutoff with the notion of DA stopping at public rating $r$.}

\begin{defn}[DA stops]
The women \emph{stop at public rating $r$} if in each woman's preference list all the edges with utility less than
$V(r,1)$
are removed. 
The women \emph{stop at man $m$} if in each woman's preference list all the edges following her edge to $m$ are removed.
The women \emph{double cut at man $m$ and public rating $r$}, if they each stop at $m$ or $r$, whichever comes first.
Men stopping and double cutting are defined similarly. Finally, an edge is said to \emph{survive} the cutoff if it is not removed by the stopping.
\end{defn}

\rjc{To obtain our bounds for man $m_i$, we will have the women double cut at rating $r_{m_i}-\alpha$ and at man $m_i$, where $\alpha>0$ is a parameter we will specify later.}

Our upper bounds in all of the utility models depend on a parameterized key lemma (Lemma \ref{lem::key_bounded}) stated shortly.
This lemma concerns the losses the men face in the woman-proposing DA; a symmetric result applies to the women.
The individual theorems follow by setting the parameters appropriately.
Our key lemma uses three parameters:
$\alpha,\beta,\gamma >0$. 
To avoid rounding issues, we will choose $\alpha$ so that $\alpha n$ is an integer.
The other parameters need to satisfy the following constraints.
\begin{align}
\label{eqn::beta-constraint}
   &\text{for $r\ge \alpha$:}\hspace*{0.5in} V(r-\alpha,1) \le V(r,1-\beta)\\
    \label{eqn::gamma-constraint}
    &\text{for $r\ge 3\alpha$:}\hspace*{0.5in} U(r,1) - U(r-3\alpha,1-\gamma)\le L
    \end{align}
\rjc{Equation~\eqref{eqn::beta-constraint} relates the range of private values that will yield a woman
an edge to $m_i$ that survives the cut at $r_{m_i} - \alpha$, or equivalently the probability of having such an edge.
Observation~\ref{obs::towards-man-accept} below, shows that Equation~\eqref{eqn::gamma-constraint} identifies
the range of $m_i$'s private values for proposals from $\widetilde{W}_i$ that yield him a loss of at most $L$
(for we will ensure the women in $\widetilde{W}_i$ have public rating at least $r_{w_i} - 3\alpha$).
}

\begin{obs}
\label{obs::towards-man-accept}
Consider the proposal from woman $w$ to the rank $i$ man $m_i$.
Suppose the rank $i$ woman $w_i$ has rating $r_{w_i}\ge 3\alpha$.
If $w$ has public rating $r\ge r_{w_i}-3\alpha$ and $m_i$'s private score for $w$ is at least $1-\gamma$,
then $m_i$'s utility for $w$ is at least $U(r_{w_i}-3\alpha,1-\gamma)\ge  U(r_{w_i},1)-L$.
\end{obs}

In the linear separable model with $\lambda = \tfrac 12$, we set $\alpha=\beta=\gamma$ and $L=2\alpha$.

The next lemma determines the probability that man $m_i$ receives a proposal 
\rjc{causing him a loss of at most $L$.}
% providing utility at least $U(r_{w_i},1)-L$, i.e.\ a loss of at most $L$. 
The lemma calculates this probability in terms of the parameters we just defined. Note that the result does not depend on the utility functions $U(\cdot,\cdot)$ and $V(\cdot,\cdot)$ being linear. In fact, the same lemma applies to much more general utility models which we also study (see Section~\ref{sec::utility_models}) and it is the crucial tool we use in all our upper bound proofs.

In what follows, to avoid heavy-handed notation, by
$r_{m_i}-\alpha$ we will mean $\max\{0,r_{m_i} - \alpha\}$.

\rjc{In order to state our next result crisply}, we define the following Event ${\cal E}_i$.
It concerns a run of woman-proposing DA with double cut at the rank $i$ man $m_i$ 
and at public rating $r_{m_i} - \alpha$. 
Let $h_i=\big|M[r_{m_i} - \alpha,1]\big| - i$,
$\ell_i = h_i + \alpha n -1$, and
$\overline{w}_i$ be the woman with rank $i+\ell_i$.
Event ${\cal E}_i$ occurs if \rjc{$i+\ell_i \le n$} and
% $\overline{w}_i$ exists and
between them the $i+\ell_i$ women in $W[r_{\overline{w}_i},1]$ make at least one proposal to $m_i$ that 
\rjc{causes him a loss of at most $L$.}
% provides him utility at least $U(r_{w_i},1)-L$.
\RJC{Could we replace $r_{\overline{w}_i}$ with $r_{w_i} - 3\alpha$? This would slightly simplify the statements of our results.}

Finally we define Event $\cal E$: it happens if ${\cal E}_i$ occurs for all $i$ such that $r_{w_i}\ge 3\alpha$.

\begin{lemma}\label{lem::key_bounded}
Let $\alpha>0$ and $L>0$ be given, and suppose that $\beta$ and $\gamma$ satisfy
\eqref{eqn::beta-constraint} and \eqref{eqn::gamma-constraint}, respectively.
Then, Event $\cal E$ occurs with probability at least $1-p_f$,
where the failure probability 
$$p_f=n\cdot \exp(-\alpha(n-1)/12)
+n\cdot \exp(-\alpha n/24)
    +n\exp(-\alpha\beta n/8)
%    +2n\cdot exp(-5\alpha^2 n/24)
    +n\cdot \exp(-\alpha\beta\gamma n/2).$$
\hide{
${cal E}$ is the occurrence of 
For Event ${\cal E}_i$, %Suppose that 
woman-proposing DA is run with double cut at the rank $i$ man $m_i$ 
and public rating $r_{m_i} - \alpha$. 
Let $h_i=\big|M[r_{m_i} - \alpha,r_{m_i}]\setminus\{m_i\}\big|$,
$\ell_i = h_i + \alpha n -1$, and
$\overline{w}_i$ be the woman with rank $i+\ell_i$.
Event ${\cal E}_i$ occurs if
$\overline{w}_i$ exists and
between them the $i+\ell_i$ women in $W[r_{\overline{w}_i},1]$ make at least one proposal to $m_i$ that provides him utility at least $U(r_{w_i},1)-L$.
}
\end{lemma}
%
\hide{
We are considering an interval of men descending
from man $m_i$ covering a public rating range of length
$\alpha$. Suppose there are $h_i$ men in this interval.
We are also considering an interval of $\ell_i$ women 
descending from $w_i$, where $\ell_i =h_i+\alpha n -1$.
(See Fig.~\ref{fig::key_bounded}.)
}
%
The following simple claim notes that the men's loss when running the full DA is no larger than when running double-cut DA.

\begin{claim}
\label{clm::full-DA-better}
Suppose a woman-proposing double-cut DA at man $m_i$ and rating $r$ is run, and suppose $m_i$ incurs a loss of $L$.
Then in the full run of woman-proposing DA, $m_i$ will incur a loss of at most $L$.
\end{claim}
\begin{proof}
Recall that when running the women-proposing DA the order in which unmatched women are processed does not affect the outcome.
Also note that as the run proceeds, whenever a man's match is updated, the man obtains an improved utility.
Thus, in the run with the full edge set we can first use the edges used in the double-cut DA and then proceed with 
the remaining edges.
Therefore if in the double-cut DA $m_i$ has a loss of $L$,
in the full run $m_i$ with have a loss of at most $L$.
\end{proof}

To illustrate how this lemma is applied, we now prove
Theorem~\ref{thm::basic-linear-result}.

\begin{proof} (Of Theorem~\ref{thm::basic-linear-result})~
By Lemma~\ref{lem::key_bounded}, in the double-cut DA, 
for all $i$ with $r_{w_i}\ge 3 \alpha$,
$m_i$ obtains a match giving him loss at most $\Lbar$,
with probability at least
$1-n\cdot \exp(-\alpha(n-1)/12)
-n\cdot \exp(-\alpha n/24)
% +2n\cdot exp(-5\alpha^2 n/24)
    -n\exp(-\alpha^2 n/8)
    -n\cdot \exp(-\alpha^3 n/2)$.

By Claim~\ref{clm::full-DA-better}, $m_i$ will incur at most a loss of $\Lbar$ in the full run of woman-proposing DA with at least as large a probability.
But this is the man-pessimal match. Consequently, in every stable match,
$m_i$ has a loss of at most $\Lbar$. 
By symmetry, the same bound applies to each woman $w_i$ such that $r_{m_i}\ge 3\alpha$.

We choose $\Lbar = [16(c+2)\ln n/n]^{1/3}$. \rjc{Recalling that $\alpha=\Lbar/2$, we see that} for large enough $n$ the probability bound, over all the men and women, is at most $1-n^{-c}$.
%
The bounds $r_{w_i}\ge 3\alpha$ and $r_{m_i}\ge 3\alpha$ imply we can set $\sigmabar=3\alpha =\tfrac 32\Lbar$.
\end{proof}

\hide{
We now outline the main ideas used in the proof of Lemma \ref{lem::key_bounded}. Our task is to prove that each individual man $m_i$ (outside the bottom-most men) gets a proposal from a woman in $W[r_{\overline{w}_i},1]$ which yields him less than $L$ loss, with high probability; we can then use a union bound to prove the lemma. To do this we consider a run of woman-proposing DA, but we focus on the women in $W[r_{\overline{w}_i},1]$ and we examine the proposals made in the following particular order: we have the women propose, in their order of preference, up to $m_i$, however they do not make proposals yielding them utility $V(r_{m_i}-\alpha,1)$ or lower. We would like to say that since we have women from $W[r_{\overline{w}_i},1]$ proposing, and they are proposing to roughly $\alpha n$ fewer men, thus there are $\alpha n$ `extra women' who must remain unmatched throughout this portion of the run of DA. Since each of these women has at least a $\beta$ chance to propose to $m_i$, we get, by a simple Chernoff bound, a guarantee that $m_i$ will receive at least $(1/2)\alpha\beta n$ proposals (the half being just a factor lost due to the Chernoff bound). Each such proposal has at least a $\gamma$ chance of being `good enough' (less than $L$ loss) for $m_i$, which gives us the result for $m_i$ with an $\exp(\alpha\beta\gamma n/2)$ probability. We can then set the parameters $\alpha$, $\beta$ and $\gamma$ so that this suffices.   

However, the major complicating feature is that while we argued above that there are at least $\alpha n$ unmatched women at each step, these may not be the same $\alpha n$ women throughout the process. Thus, to complete our argument, we prove that in fact the worst case scenario for us is when the $\alpha n$ women are the same throughout, which is the case we are able to analyze.
}

\begin{proof} (Of Lemma \ref{lem::key_bounded}. Sketch.)
We run the double-cut DA in two \rjc{phases}, defined as follows. 
Recall that $h_i=\big|M[r_{m_i}-\alpha,r_{m_i}]\setminus\{m_i\}\big|$ and $\ell_i=h_i+\alpha n-1$.
\\
\emph{Phase 1}. Every unmatched woman with rank at most
$i+\ell_i$ 
keeps proposing until her next proposal
is to $m_i$,
or she runs out of proposals.\\
\emph{Phase 2}. Each unmatched women makes her next proposal, if any, which will be a proposal to $m_i$.

\smallskip
In this sketch we will be using the term with high probability (w.h.p.) to mean
with probability at least $1-n^{c+2}$.

Our analysis is based on the following four observations. The first two are simply observations that w.h.p.\ the number of agents with
public ratings
in a given interval is close to the
expected number. We defer the details to the appendix.

A critical issue in this analysis is to make sure the conditioning induced by the successive steps of the analysis does not affect the independence needed for subsequent steps. To achieve this, we use the Principle of Deferred Decisions, only instantiating
random values as they are used.
Since each successive bound uses a different collection of random variables this does not present a problem.

\smallskip
\noindent
i. 
% Let $h_i=\big|M[s_{m_i}-\alpha,s_{m_i}]\setminus\{m_i\}\big|$.
As $\text{E}[h_i] =\alpha(n-1)$,
w.h.p.,
$h_i \le \tfrac 32 \alpha (n-1)$.
This claim uses a Chernoff bound with the randomness coming from
the public ratings 
of the men.

\smallskip
\noindent
ii. Assuming the high probability event in (i),
% by Claim~\ref{clm::span-woman-interval}, 
w.h.p.,
This claim uses a Chernoff bound 
with the randomness coming from the public ratings of the women.

\hide{
\smallskip
\noindent
iii. w.h.p., for all $i$, $s_{m_i} < s_{w_i} +\alpha$. This follows by showing that w.h.p.\ there are fewer than $i$ men in $M[(1-\tfrac in)+\tfrac12 \alpha,1]$ and
more than $i$ women in $W[(1-\tfrac in)-\tfrac12 \alpha,1]$; so $s_{m_i}<(1-\tfrac in)+\tfrac12 \alpha$
and $s_{w_i}>(1-\tfrac in)-\tfrac12 \alpha$,
and therefore $s_{m_i} < s_{w_i} +\alpha$.
these w.h.p.\ claims apply Chernoff bounds
based on the public ratings %values 
of the men and women.
}

\smallskip
\noindent
iii. w.h.p., between them, the women with
rank at most $i+\ell_i$ make at least
$\tfrac 12 \alpha\beta n$ Phase 2 proposals to $m_i$.
This bound uses the private scores of the women
and uses a novel argument \rjc{to sidestep the conditioning
among these proposals}. %we discuss below.

\smallskip
\noindent
iv. Assuming the high probability events in (i)--(iii),
at least one of the Phase 2 proposals to $m_i$ will
provide him utility at least $U(r_{w_i},1)-L$ with probability at least
$1 -(1-\gamma)^{\alpha\beta n/2}\ge 1 -\exp(\alpha\beta\gamma n/2)$.
The randomness comes from the private scores of the men.

To see this, note that each Phase 2 proposal is from a woman $w$ with rank at most $i+\ell_i$. 
By (ii), her public rating is at least $r_{w_i} -3\alpha$. 
Recall that man $m_i$'s utility for $w$ equals
$U(r_w,s_{m_i}(w))\ge U(r_{w_i}-3\alpha,s_{m_i}(w))$.
To achieve utility at least $U(r_{w_i},1)-L \le U(r_{w_i}-3\alpha,1-\gamma)$ (using \eqref{eqn::gamma-constraint}) it suffices to have
$s_{m_i}(w) \ge 1-\gamma$, which happens with
probability $\gamma$.
Consequently, utility at least $U(r_{w_i},1)-L$ is
achieved with probability at least $\gamma$.

For each Phase 2 proposal these probabilities are independent as they reflect $m_i$'s private
scores for each of these proposals.
%
%Thus the Step 2 proposals (weakly) stochastically dominate a collection of $\tfrac 12 \alpha\beta n$ proposals to $m_i$ each having probability $\gamma$ of providing utility $U(s_{w_i},1)-L$ or more.
Therefore the probability that there is no proposal providing $m_i$ a loss of at most $L$ is at most 
\begin{align*}
    \big(1-\gamma\big)^{\alpha\beta n/2}\le \exp(\alpha\beta\gamma n/2).
\end{align*}
\end{proof}



% We choose $\Lbar = [16(c+2)\ln n/n]^{1/3}$, and then the bound becomes at most $n^{-(c+2)}$.


We return to justifying (iii).

First, we simplify the action space by viewing the decisions as being made on a discrete utility space.
We do this in such a way that for each woman the probability of selecting $m_i$ is only increased,
and the probability of having any differences
in the sequence of actions in the original continuous setting and the discrete setting is at most $\delta$.
We detail how to construct this discrete utility space
in the appendix. The space will depend on
$\delta$, which can be arbitrarily small. 

We represent the possible computations of the double-cut DA in this discrete setting using a tree $T$. Each woman will be going through her possible utility values in decreasing order, with the possible actions of the various women being interleaved in the order given by the DA processing.
Each node $u$ corresponds to a woman $w$ processing her next utility value: the possible choices at this utility, each represented by an edge descending from $u$, are:

i. Proposing to some man 
(among those men $w$ has not yet proposed to); or 

ii. ``no action''. This corresponds 
to $w$ making no proposal achieving the current utility.

\noindent
We observe the following important structural feature of tree $T$.
Let $S$ be the subtree descending from the edge corresponding to woman $w$ proposing to $m_i$;
in $S$ there are no further actions of $w$, i.e.\ no nodes at which $w$ makes a choice, because \rjc{the double cut} DA cuts at the proposal to $m_i$.

At each leaf of $T$, up to 
$i+h_i -1= i+\ell_i - \alpha n$
%$i+\ell_i - \alpha n$ 
women will have been matched with someone other than $m_i$
(recall that $\ell_i =h_i + \alpha n - 1$).
%, because $\big|W[r_{\overline{w}},1]\big| - \big|M[r_{m_i},1]\setminus\{m_i\}\big|=(i+\ell_i)-(i+h_i-1)=(h_i+\alpha n -1) - (h_i-1) =\alpha n$. 
The other women either finished with a proposal to $m_i$ or both failed to match and did not propose to $m_i$. Let $w$ be a woman in the latter category.
Then, 
on the path to this leaf, $w$ will have traversed edges corresponding to a choice at each discrete utility in the range $[V(r_{m_i}-\alpha,1),V(1,1)]$.


We now create an extended tree, $T_x$, by adding a subtree at each leaf; this subtree will correspond to pretending there were no matches; the effect is that % i.e.\ 
each women will take an action at all their remaining utility values in the range
$[V(r_{m_i}-\alpha,1),V(1,1)]$,
except that in the sub-subtrees descending from edges that correspond to some woman $w$ selecting $m_i$, $w$ has no further actions.
For each leaf in the unextended tree, the probability
of the path to that leaf is left unchanged.
The probabilities of the paths in the extended tree are then calculated by multiplying the path probability in the unextended tree with the probabilities of each woman's choices in the extended portion of the tree.

Next, we create an artificial mechanism $\mathcal M$ that acts on tree $T_x$. The mechanism $\mathcal M$
is allowed to put $i+\ell - \alpha n$ ``blocks'' on each path; blocks can be placed at internal nodes. A block names a woman $w$ and corresponds to her matching (but we no longer think of the matches as corresponding to the outcome of the edge selection; they have no meaning beyond making
all subsequent choices by this woman be the ``no action'' choice).

DA can be seen as choosing to place up to $i+\ell - \alpha n$ blocks at each of the nodes corresponding to a leaf of $T$.
$\mathcal M$ will place its blocks so as to minimize the probability $p$ of paths with at least $\tfrac12 \alpha\beta n$ women choosing edges to $m_i$.
Clearly $p$ is a lower bound on the probability
that DA makes at least $\tfrac12 \alpha\beta n$ proposals in Phase 2.
Given a particular choice of blocks, we call the resulting probability of having fewer than $\tfrac12 \alpha\beta n$ women choosing edges to $m_i$, the \emph{blocking probability}.



\begin{claim}
\label{clm::many-props-despite-blocking}
The probability that $\mathcal M$ makes at least $\tfrac 12\alpha\beta n$ proposals to $m_i$ is at least $1-\exp(-\alpha\beta n/8)$.
\end{claim}
\begin{proof}
We will show that the most effective blocking strategy is to block all but $\alpha n$ women before they have made any choices.
Then, the remaining $\alpha n$ women all have independent probability at least $\beta$ of making a proposal to $m_i$.
In expectation, there are at least $\alpha\beta n$ proposals to $m_i$, and therefore, by a Chernoff bound,
at least $\tfrac 12 \alpha\beta n$ proposals with probability at least $1-\exp(-\alpha\beta n/8)$.

The claim about the best blocking strategy follows
by showing that at a node $x$ such that the only blocks below it are at its children, the blocks, possibly modified, can be moved to $x$. This requires a case analysis, deferred to the appendix. Iterating the argument demonstrates the claim.
\end{proof}

\begin{cor}
\label{cor::many-props-to-m-mtm}
The probability that the double-cut DA makes at least $\tfrac 12\alpha\beta n$ proposals to $m_i$ is at least $1-\exp(-\alpha\beta n/8)$.
\end{cor}
\begin{proof}
For any fixed $\delta$, by Claim~\ref{clm::many-props-despite-blocking}, the probability that $\mathcal M$ makes at least $\tfrac 12\alpha\beta n$ proposals to $m_i$ is at least $1-\exp(-\alpha\beta n/8)$.
By construction, the probability is only larger for the double-cut DA in the discrete space.

Therefore, by Claim~\ref{clm::full-DA-better}, the probability that the double-cut DA makes at least $\tfrac 12\alpha\beta n$ proposals to $m_i$ in the actual continuous space is at least $1-\exp(-\alpha\beta n/8)-\delta$, and this holds
for any $\delta>0$, however small.
Consequently, this probability is at least $1-\exp(-\alpha\beta n/8)$.
\end{proof}








==> other-related-work1.tex <==

\section{Other Related work}
\label{sec::other-related}

The random preference model was introduced by Knuth~\cite{Knuth76} (for a version in English see~\cite{Knuth96}), and subsequently extensively analyzed~\cite{Pittel89,KMRP90,Pittel92,Mertens05,PSV07,Pittel18,Kupfer20}.
In this model, each agent's preferences are an independent uniform random permutation of the agents on the other side.
An important observation was that when running the DA algorithm, the rank of preferences obtained by proposing side was $\Theta(\ln n)$ on the average,
but on the other side it was $\Theta(n/\ln n)$.

A recent and unexpected observation 
% by Ashlagi, Kanoria and Leshno
in~\cite{AKL17} was the
``stark effect of competition'': that in the random preferences model the short side, whether it was the proposing side or not, was the one to enjoy the $\Theta(\ln n)$ rank matches.
Subsequent work
% Kanoria, Min and Qian~\cite{KanoriaMinQian21}
showed that
this effect disappeared with short preference lists
in a natural modification of the random preferences model~\cite{KMQ21}.
Our work suggests yet another explanation for why this effect may not be present: it does not require that short preference lists be imposed as an external constraint, but rather that the preference model generates few edges that might ever be in a stable matching.

% Coming back to Lee's work, his main result was to show that as the market size increases, the incentive to misreport preference lists shrinks, where the incentive is measured in terms of expected gain in utility.
%  His analysis used a simple benchmark --- the public rating assortative match: suppose the men and women were each ordered based on decreasing public ratings, with $m_i$ being the $i$th man in this ordering and $w_i$ the $i$th woman; also let $r_{m_i}$ denote $m_i$'s public score. The benchmark utility woman $w_i$ seeks is defined to be $\tfrac12 (r_{m_i} +1)$, i.e.\ the utility she would obtain if she were matched with $m_i$ and her private score for $m_i$ was the maximum possible. The men's benchmark utilities are defined in the same way.

% Lee's result states that, with high probability, every stable
% matching has the following property: Given constants $\sigma,\eps>0$, for large enough $n$,
% apart from a $\sigma$ fraction of the women, every other woman will obtain a match having utility at most $\eps$ smaller than her benchmark,
% and similarly for the men. In fact, Lee showed this result for a much wider class of utility functions.

The number of edges present in any stable matching has also been examined for a variety of settings. When preference lists are uniform the expected number of stable pairs is $\Theta(n\ln n)$~\cite{Pittel92}; when they are arbitrary on one side and uniform on the other side, the
expected number is $O(n\ln n)$~\cite{KMRP90}. This result
continues to hold when preference lists
are arbitrary on the men’s side and are generated from general popularities on the women’s side~\cite{GMM19}. Our analysis shows that in the linear separable model (and more generally in the bounded derivative setting) the expected number of stable pairs is also $O(n\ln n)$.

Another important issue is the amount of communication needed to identify who to place on one's preference lists
when they have bounded length. In general, the cost is $\Omega(n)$ per agent (in an $n$ agent market)~\cite{GNOR15},
but in the already-mentioned separable model of Ashlagi et al.\ \cite{ABKS19} this improves to $O^*(\sqrt{n})$
given some additional constraints, and further improves to $O(\ln^4n)$ in a tiered separable market~\cite{ABKS19}.
We note that for the bounded derivatives setting, with high probability, the communication cost will be
$O(n^{1/3}\ln^{2/3}n)$ for all agents except the bottommost $\Theta(n^{2/3}\ln^{1/3} n)$,
for whom the cost can reach $O(n^{2/3}\ln^{1/3} n)$.

Another approach to selecting which universities to apply to was considered by Shorrer who devised a dynamic program to compute the optimal choices for students assuming universities had a common ranking of students~\cite{Shorrer19}.

==> prelim.tex <==
\section{Preliminaries} \label{sec::prelim}

\subsection{Stable Matching and the Deferred Acceptance (DA) Algorithm}


Let $M$ be a set of $n$ men and $W$ a set of $n$ women. Each man $m$ has an ordered list of women that represents his preferences, i.e.\ if a woman $w$ comes before a woman $w'$ in $m$'s list, then $m$ would prefer matching with $w$ rather than $w'$. 
The position of a woman $w$ in this list is called $m$'s ranking of $w$. Similarly each woman $w$ has a ranking of her preferred men\footnote{Throughout this paper, we assume that each man $m$ (woman $w$) ranks all the possible women (men), i.e.\ $m$’s ($w$’s) preference list is complete.}. The stable matching task is to pair (match) the men and women in such a way that no two people prefer each other to their assigned partners. More formally:

\begin{defn}[Matching]
A matching is a pairing of the agents in $M$ with the agents in $W$.
It comprises a bijective function $\mu$ from $M$ to $W$, and its inverse
$\nu=\mu^{-1}$, which is a bijective function from $W$ to $M$. 
\end{defn}

\begin{defn}[Blocking pair]
A matching $\mu$ has a blocking pair $(m,w)$ if and only if: %the following conditions are all met:
%
\begin{enumerate}
    \item $m$ and $w$ are not matched: $\mu(m)\neq w$.
    \item $m$ prefers $w$ to his current match $\mu(m)$.
    \item $w$ prefers $m$ to her current match $\nu(w)$. % $\mu^{-1}(w)$.
\end{enumerate}
\end{defn}

\begin{defn}[Stable matching]
A matching $\mu$ is stable if it has no blocking pair.
\end{defn}
\begin{algorithm}[t]
\SetAlgoNoLine
Initially, all the men and women are unmatched.\\
\While{some woman $w$ with a non-empty preference list is unmatched}{ 
   let $m$ be the first man on her preference list\;
   \If{$m$ is currently unmatched}
      {tentatively match $w$ to $m$.}
      {\eIf{$m$ is currently matched to $w'$, and $m$ prefers $w$ to $w'$}
      {make $w'$ unmatched and tentatively match $w$ to $m$.}
      {remove $m$ from $w$'s preference list}
    }
 }
\caption{\textsf{Woman Proposing Deferred Acceptance (DA) Algorithm.}}
\label{alg:DA}
\end{algorithm}

Gale and Shapley \cite{GS} proposed the seminal deferred acceptance (DA) algorithm for the stable matching problem. We present the woman-proposing DA algorithm (Algorithm $1$); the man-proposing DA is symmetric.
%
The following facts about the DA algorithm are well known. We state them here without proof and we shall use them freely in our analysis. 

\begin{obs}
\hspace{0.0001in}
\begin{enumerate}
    \item \label{obs::DA_terminates_in stable_match}
DA terminates and outputs a stable matching.
\item\label{obs::DA_invariant_of_proposal_order}
The stable matching generated by DA is independent of the order in which the unmatched agents on the proposing side are processed.
\item\label{obs::DA_optimality}
Woman-proposing DA is woman-optimal, i.e.\ each woman is matched with the best partner she could be matched with in any stable matching.
\item \label{obs::DA_pessimality}
Woman-proposing DA is man-pessimal, i.e.\ each man is matched with the worst partner he could be matched with in any stable matching.
\end{enumerate}
\end{obs}



\subsection{Useful notation and definitions}

There are $n$ men and $n$ women.
In all of our models, each man $m$ has a utility $U_{m,w}$ for the woman $w$, and each woman $w$ has a utility $V_{m,w}$ for the man $w$. These utilities are defined as
\begin{align*}
    &U_{m,w}=U(r_w,s_m(w)), \text{ and}\\
    &V_{m,w}=V(r_m,s_w(m)),
\end{align*}
where $r_m$ and $r_w$ are common public ratings, $s_m(w)$ and $s_w(m)$ are private scores specific to the pair $(m,w)$, and $U(\cdot,\cdot)$ and $V(\cdot,\cdot)$ are continuous and strictly increasing functions from $\mathbb{R}^2_+$ to $\mathbb{R}_+$.
The ratings are independent uniform draws from $[0,1]$ as are the scores.

In the \emph{Linear Separable Model},
each man
$m$ assigns each woman $w$ a utility of $U_{m,w}=\lambda\cdot r_w+(1-\lambda)\cdot s_m(w)$, where $0< \lambda < 1$ is a constant.
The women's utilities for the men are defined analogously as $V_{m,w}=\lambda\cdot r_m+(1-\lambda)\cdot s_w(m)$.
% Here we assume both public ratings and private scores are drawn uniformly from $[0,1]$.
All our experiments are for this model.

We let $\{m_1, m_2, \ldots, m_n\}$ be the men in descending order of their public ratings and $\{w_1, w_2, \ldots, w_n\}$ be a similar ordering of the women. 
We say that $m_i$ has public rank $i$, or rank $i$ for short,
and similarly for $w_i$.
We also say that $m_i$ and $w_i$ are \emph{aligned}.
In addition, we often want to identify the men or women in an interval of public ratings.
Accordingly, we define $M(r,r')$ to be the set of men with public ratings in the range $(r,r')$,
and $M[r,r']$ to be the set with public ratings in the range $[r,r']$; we also use the notations
$M(r,r']$ and $M[r,r')$ to identify the men with ratings in the corresponding semi-open intervals.
We use an analogous notation, with $W$ replacing $M$, to refer to the corresponding sets of women.

We will be comparing the achieved utilities in stable matchings to the following benchmarks: the rank $i$ man has as benchmark $U(r_w,1)$,
the utility he would obtain from the combination of the rank $i$ woman's public rating and the highest possible private score;
and similarly for the women.
Based on this we define the loss an agent faces as follows.

\begin{defn} [Loss]
\label{defn::loss_linear} 
Suppose man $m$ and woman $w$ both have rank $i$.
The \emph{loss} $m$ sustains from a match of utility $u$ is defined to be $U(r_w,1) - u$.
The loss for women is defined analogously.
\end{defn}

In our analysis we will consider a complete bipartite graph whose two sets of vertices correspond to the men and women, respectively. For each man $m$ and woman $w$, we view the possible matched pair $(m,w)$ as an edge in this graph. Thus, throughout this work, we will often refer to edges being proposed, as well as edges satisfying various conditions.

\hide{
There are $n$ men and $n$ women. 
Each man $m$ has a public rating $r_m$ and each women $w$ has a public rating $w$. These are uniform draws from $[0,1]$.

The utilities of the agents for each other are based on the public rankings and individual adjustments called scores.
Each woman $w$ has a score $s_w(m)$ for each man $m$;  likewise, each man $m$ has a score $s_m(w)$ for each woman $w$.
The scores are draws from $[0,1]$.}

==> results.tex <==
\section{Results}
\label{sec::results}
\paragraph{The Bounded Derivatives Model}
We begin by stating our basic result for this model.
%
\begin{theorem}\label{thm:basic-bdd-deriv-result}
In the bounded derivatives model, when there are $n$ men and $n$ women,
for any given constant $c>0$, for large enough $n$, with probability at least $1-n^{-c}$, in every stable match,
for every $i$, if $r_{w_i}\ge \sigmabar\triangleq 3\Lbar/4\mu$, 
% every agent,  except possibly those with public score less than $\sigmabar = \Lbar/\mu$, 
agent $m_i$ suffers a loss of at most $\Lbar$, where $\Lbar=\Theta((\ln n/n)^{1/3})$,
and similarly for the agents $w_i$.
\end{theorem}
Note that w.h.p., the public ratings of aligned agents are similar.

In words, w.h.p., all but the bottommost agents (those whose aligned agent has public rating less than $\sigmabar$) suffer a loss of no more than $\Lbar$. We call this high probability outcome $\mathcal E$.

By Theorem \ref{lem::acceptable-suffice}, the implication is that w.h.p.\ a woman can safely restrict her proposals to her acceptable edges, or to any overestimate of this set of edges obtained by her setting an upper bound on the loss she will accept from a match.
There is a small probability--- at most $n^{-c}$---that this may result in a less good outcome, namely the probability
that $\mathcal E$ does not occur.

Then,
w.h.p., every stable match gives each woman $w$, whose aligned agent $m$ has public rating $r_m\ge\sigmabar=\Omega((\ln n/n)^{1/3})$, a partner with public rating in the range $[r_m - \Lbar/\mu, r_m+ 5/4 \Lbar/\mu]$ (see appendix \ref{sec::cone-size}). An analogous statement applies to the men. 

This means that if we are running woman-proposing DA, each of these women might as well limit her proposals to her woman-acceptable edges, which is at most the men with public ratings in the range $r_m \pm \Theta(\Lbar)$ for whom she has private scores of at least $1 - \Theta(\Lbar)$. In expectation, this yields $\Theta(n^{1/3}(\ln n)^{2/3})$ men to whom it might be worth proposing. It also implies that a woman can have a gain of at most $\Theta(\Lbar)$ compared to her target utility.

If, in addition, each man can inexpensively signal the women who are man-acceptable to him, then the women can further limit their proposals to just those men providing them with a signal; in the case of accurate signals, this reduces the expected number of proposals these women can usefully make to just $\Theta(\ln n)$.


Our next result provides a distribution bound on the losses. It states that for most agents, the losses are at most
$\Theta(\Lbar/(\ln n)^{1/3})$, with a geometrically decreasing number of agents facing larger losses.

\begin{theorem}\label{thm::distr-bound}
In the bounded derivatives model, when there are $n$ men and $n$ women,
for any given constant $c>0$, for large enough $n$, with probability at least $1-n^{-c}$, in every stable match,
among the agents whose aligned partner has public score at least $\sigmabar\triangleq 3\Lbar/4\mu$, 
at most $2n\cdot\exp(-(c+2)\ln n/2^{3h})$ men suffer a loss of more
than $\Lbar/2^h$, for integer $h$ with
$\frac 13 \log\Big(\frac{(c+2)\ln n}{\ln[n/3(c+2)\ln n]}\Big) \le h \le \frac 13 \log[(c+2)\ln n]$,
and likewise for the women.
\end{theorem}


We now generalize Theorem~\ref{thm:basic-bdd-deriv-result} to possibly unequal numbers of men and women, and also state what can be said for agents with low public ratings.
%
\begin{theorem}\label{thm::low_loss_bounded}
Suppose there are $p$ men and $w$ woman, with $p\ge n$.
Let $t\ge 1$ be a parameter.
In the bounded derivatives model,
for any given constant $c>0$, for large enough $n$, with probability at least $1-n^{-c}$,
in every stable match, every agent, except possibly the 
men whose aligned agents have public rating less than $\tfrac{p-n}{n}+\tfrac{\sigmabar}{t}$ and the women
whose aligned agents have public rating less than $\tfrac{\sigmabar}{t}$, suffers a loss of at most $\Lbar t^2$, where $\Lbar =\Theta((\ln n/n)^{1/3})$
and $\sigmabar = 3\Lbar/4\mu$.
\end{theorem}
Note that when $L=1$ (i.e.\ 100\% loss), $t=\Theta((n/\ln n)^{1/6})$ and therefore $\sigmabar/t = \Theta((\ln n)/n)^{1/2})$,
providing a lower bound on the range for which this result bounds the loss.

Setting $t=1$ and $p=n$ yields Theorem~\ref{thm:basic-bdd-deriv-result}.

The implication is similar to that for Theorem~\ref{thm:basic-bdd-deriv-result},
but as $t$ increases, i.e., for women whose aligned agents have increasingly low public ratings,
the bound on the number of proposals she can usefully make grows by roughly a $t^2$ factor.

\paragraph{$\eps$-Bayes-Nash Equilibrium}


\begin{defn} \label{def::strong-bdd-deriv}
A function $f(x,y):{\mathbb R}^2\rightarrow {\mathbb R}^+$ has \emph{$(\rho_{\ell},\rho_u,\mu_{\ell},\mu_u)$-bounded derivatives} if for all $(x,y)\in {\mathbb R}^2$,
\begin{align*}
   &\text{\rm The ratio bound:}~~\rho_{\ell} \le\pdv{f}{x}\Big/\pdv{f}{y}\le \rho_u.\\ 
&\text{\rm The first derivative bound:}~~\mu_{\ell}\le \pdv{f}{x}\leq \mu_u.
\end{align*}
Then $f$ is said to have the \emph{strong bounded derivative} property. Note that in the linearly separable model,
$\rho_{\ell}=\rho_u$ and $\mu_{\ell}=\mu_u$.
\end{defn}


Let $t\geq 1$ be a parameter and $\sigmabar= \Theta([\ln n/n]^{1/3})$. Define. $L^m_t\triangleq U(r_w,1) - U(r_w-\sigmabar t^2,1)$ and
$L^w_t\triangleq V(s_m,1) - V(r_m-\sigmabar t^2,1)$. For this to be meaningful when $r_w-\sigmabar t^2 < 0$, we extend the definition of $U$ to this domain as follows. For $s<0$, $\pdv{U(r,s)}{r}=\mu_{\ell}$ and
$\pdv{U(r,s)}{s}=\rho_{\ell}$.
We proceed analogously to handle the case that
$r_m-\sigmabar t^2 < 0$. 
Define parameters $\sigma_m = \beta/ n^{1/3}$ and $\sigma_w=\nu/n^{1/3}$, where $\beta>1$ and $\nu<1$ are constants. We then define $t_m= \sigmabar/\sigma_m$ and $t_w= \sigmabar/\sigma_w$.
Note that in the strongly bounded derivatives model, $L^m_{t_m} \le \Theta\Big(\frac{\mu_u}{\beta^2}\cdot \frac{\ln n}{n^{1/3}}\Big)$ and $L^w_{t_w} \le \Theta\Big(\frac{\mu_u}{\nu^2}\cdot \frac{\ln n}{n^{1/3}}\Big)$.


\begin{theorem}\label{thm::eq-BN}
Let $\eps=\Theta(1/n^{1/3})$. There are constants $\beta>1$ and $\nu<1$ such that in the strongly bounded derivatives model, there exists an $\eps$-Bayes-Nash equilibrium where, with probability a least $1-n^{c}$, agents with public ratings greater than $\sigmabar$ make at most $\Theta(\ln n)$ proposals and all agents make at most $\Theta(\ln^2 n)$ proposals. Furthermore, in this equilibrium, with probability a least $1-n^{c}$, every man has a loss of at most $L^m_{t_m}$, and every woman $w$ has a loss of at most $L^w_{t_w}$.
\end{theorem}


\paragraph{The General Utilities Model}
\label{sec::general}
\begin{theorem}\label{thm::low_loss_general}
Let $0<\eps<1$, $0 < \sigma < 1$, and $c>0$ be constants.
In the general utilities model, for large enough $n$,
with probability at least $1-\exp(-\Theta(n))$, 
in every stable matching, every agent, 
except possibly those whose aligned agents have public rating less than $\sigma$, suffers a loss of at most $\epsilon$.
\end{theorem}

Clearly the smaller $\eps$, the smaller the ranges of public ratings and private scores that can yield acceptable proposals; however, there does not appear to be a simple functional relationship between $\eps$ and the sizes of these ranges in this general model.

\paragraph{The Many to One Setting}
%
Next, we state our many-to-one result, expressing it in terms of the $n_w$ workers and $n_c$ companies, each having $d$ positions. 
We now have possibly different bounds

\begin{align*}
\Lbar_w &= \Theta([(\ln n_w)/n_c]^{1/3})=\Theta([(d\ln n_w)/n_w]^{1/3}), ~~~~\text{and} \\
   \Lbar_c &=\left\{\begin{array}{ll}
                    \Theta((\max\{d,\ln n_w\}/n_w)^{1/3})\hspace*{0.5in} & % d=O(\ln n_w)\\
%                    \Theta((d/n_w)^{1/3})& \Theta(\ln n_w) \le
                   d= O((n_w/\ln n_w)^{2/3})\\
                   \Theta((d\ln n_w)/n_w) & d =\Omega( n_w/\ln n_w)^{2/3})
                 \end{array}
         \right.
\end{align*}
% $\Theta([\max\{d,\ln n_w\}/n_w]^{1/3})$ 
on the losses for non-bottommost workers and companies.
Analogous to the one-to-one case, we define $\sigmabar_c = 3\Lbar_c/4\mu$ and $\sigmabar_w = 3\Lbar_w/4\mu$, the public rating thresholds below which these loss bounds need not hold.

\begin{theorem}
\label{thm::many-to-one}
Let % $r\ge 1$ be a parameter, and let 
$\Lbar_c$, $\Lbar_w$, $\sigmabar_c$ and $\sigmabar_w$ be as defined above.
Suppose that $d=O((n/\ln n)^{2/3})$.
Then, for any given constant $k>0$, with probability at least $1-n^{-k}$,
in every stable match, every company, except possibly those whose aligned agent has public rating less
than $\sigmabar_w$, suffers a loss of at most $\Lbar_c$,
and every worker, except possibly those whose aligned agent has public rating less
than $\sigmabar_c$, suffers a loss of at most $\Lbar_w$.
\end{theorem}


\paragraph{Lower Bounds}
%
The next two theorems show that the bounded derivative result is tight in two senses.
First, we show that the bound $\Lbar$ on the loss is tight up to a constant factor. 
%
\begin{theorem}
\label{thm::Lbar-bound-tight}
In the linear separable model with $\lambda = \tfrac 12$,
if $n\ge 32,000$ and $L= \tfrac 18 (\ln n/n)^{1/3}$,
then with probability at least $\tfrac 14 n^{-1/8}$ there is no perfect matching, let alone stable matching,
in which every agent with public rating $\tfrac 32 L$ or larger suffers a loss of at most $L$. (Here $\mu=\tfrac 12$, so $\tfrac 32 L=3L/4\mu.)$
\end{theorem}

Next, we show that to obtain sub-constant losses in general, one needs constant bounds on the derivatives. 
We first define a notion of a sub-constant function, which we use to specify sub-constant losses.

\begin{defn}[Sub-constant function]
A function $f(x):{\mathbb R}\rightarrow {\mathbb R}^+$ is sub-constant if for every choice of constant $c>0$, there exists an $\xbar$ such that for all $x \ge\xbar$, $f(x) \le c$.
\end{defn}

\begin{theorem}\label{thm:constant-deriv-bdd-needed}
Let $f:N\rightarrow {\mathbb R}^+$ 
be a continuous, strictly decreasing sub-constant function,
and let $\delta,\sigma \in (0,1)$ be constants. 
Then, in the following two cases, there exist continuous and strictly increasing utility functions $U(.,.)$ and $V(.,.)$ such that for some $\nbar>0$,
%for every constant $0 < \eps \le 1$,
for all $n\ge \nbar$, with probability at least $1 - \delta$, in every perfect matching, some rank $i$ man $m_i$ or woman $w_i$ with public rating at least $\sigma$ receives utility less than $U(r_{w_i},1)-f(n)$ or $V(r_{m_i},1)-f(n)$, respectively.

\smallskip

i.  $U(.,.)$ and $V(.,.)$ have derivatives w.r.t.\ their second variables that are bounded by a constant, but for (at least) one of which the derivative w.r.t.\ their first variable is not bounded by any constant.

\smallskip

ii. $U(.,.)$ and $V(.,.)$ 
have derivatives w.r.t.\ their first variables that are bounded by a constant, but for (at least) one of which the derivative w.r.t.\ their second variable is not bounded by any constant.
\end{theorem}

==> utility_models.tex <==
\section{More General Models}
\label{sec::utility_models}
\subsection{Utility Models}
\hide{
It is natural to view the men and women's ordered preference lists as arising from the fact that the agents differ regarding their perceived utility values for their possible partners. As already discussed, this topic has been %extensively 
explored in the literature, in particular in settings where these utility values are thought of as being drawn, either explicitly or implicitly, from various distributions. 
% The first such probabilistic setting to be well understood was the case where utilities are uniformly and independently drawn, and subsequently additional results have furthered our understanding in a variety of more general settings. 
We now define the utility models and settings we consider in this work.
}


\paragraph{The General Utilities Model}
There are $n$ men and $n$ women. Each man $m$ has a utility $U_{m,w}$ for the woman $w$, and each woman $w$ has a utility $V_{m,w}$ for the man $w$. These utilities are defined as
\begin{align*}
    &U_{m,w}=U(r_w,s_m(w)), \text{ and}\\
    &V_{m,w}=V(r_m,s_w(m)),
\end{align*}
where $r_m$ and $r_w$ are common public ratings, $s_m(w)$ and $s_w(m)$ are private scores specific to the pair $(m,w)$, and $U(\cdot,\cdot)$ and $V(\cdot,\cdot)$ are continuous and strictly increasing functions from $\mathbb{R}^2_+$ to $\mathbb{R}_+$.

The public ratings and private scores are drawn independently from distributions with positive density functions with bounded support on $\mathbb{R}_+$. We assume without loss of generality that all public ratings and private scores are drawn uniformly and independently from $[0,1]$ since there is always a change of variables that transforms them into uniform draws while transforming the utility functions monotonically.

$U$ and $V$ are not explicitly assumed to be bounded. However they are continuous and for the purpose of our analysis we can restrict the domain of $U$ and $V$ to the product of the bounded supports of our ratings and score distributions. These restricted $U$ and $V$ are continuous functions on a compact set and hence are bounded. Now, WLOG, by scaling appropriately, we can assume the range of $U$ and $V$ are both $[0,1]$.


\paragraph{The Bounded Derivatives Model}
We add a notion of bounded derivatives to the general utilities model.

\begin{defn} \label{def::bdd-deriv}
A function $f(x,y):{\mathbb R}^2\rightarrow {\mathbb R}^+$ has \emph{$(\rho,\mu)$-bounded derivatives} if for all $(x,y)\in {\mathbb R}^2$,
\begin{align*}
   &\rho \le\pdv{f}{x}\Big/\pdv{f}{y}~~\text{\rm --- the ratio bound};\\ 
&\pdv{f}{x}\leq \mu~~\hspace*{0.32in}\text{\rm --- the first derivative bound}.
\end{align*}
\end{defn}
Note that this definition implies $\pdv{f}{y}$ is upper bounded by $\mu/\rho$.

\smallskip

In the bounded derivatives model, the utility functions $U$ and $V$ are restricted to having $(\rho,\mu)$-bounded derivatives, for some constants $\rho, \mu > 0$. In the linear separable model, which is a special case of this model, $\mu= \lambda$ and $\rho=\lambda/(1-\lambda)$.

\subsection{Other Generalizations}

\paragraph{Unequal numbers of men and women} We generalize the above models to allow for $n$ women and $p$ men, where $n$ and $p$ need not be equal.
Suppose that $n\le p$. It is then convenient to change the public rating ranges to be $[0,p/n]$ for the men and $[p/n -1,p/n]$ for the women. We proceed symmetrically when $n>p$. We will keep the private score range at $[0,1]$. The effect of this change is to ensure that with
high probability the top $n$ public ratings for the men cover approximately the same range as the women's public ratings.

\paragraph{Many-to-one matchings} The stable matching problem has also been studied in the setting of many-to-one matchings. For example, in the setting of employees and employers, often employers want to hire multiple employees. For this setting, we will refer to the two sides as %use the language of 
companies and workers. % in our exposition.
Also, we will focus on the bounded derivatives setting.

There are $n_c$ companies and $n_w$ workers.
%$c_1,c_2\ldots,c_m$, in decreasing order of public scores. 
Each company has $d$ positions, meaning that it wants to match with $d$ workers.
%A company has a size of $d$, if it can have up to $d$ employees matched to it in the matching. 
% $d_i$ denotes the size of company $c_i$. Furthermore the company sizes are bounded; all company sizes lie in the range $[d_l,d_u]$; and $\dav$ denotes the average size of a company.
%$P(c_i)$ is the number of positions available at companies with public scores up to and including $c_i$, i.e.\ $P(c_i)=\sum_{h=1}^{i} d_h$. 
%
%There are $n$ workers.
%$w_1,w_2\ldots,w_n$, also in decreasing order of public scores. 
Each worker can be hired by only one company. The total capacity of all the companies exactly matches the number of workers, i.e.\ $n_c\cdot d=n_w$.\footnote{Our results generalize easily to the case in which the number of workers differs from the number of available positions. We omit the details.}

$r_c$ will denote the public rating of company $c$, and $r_w$ the public rating of worker $w$. Worker $w$ has private score $s_w(c)$ for company $c$, and company $c$ has private score $s_c(w)$ for worker $w$. 
$U(r_w,s_c(w))$ denotes the utility company $c$ has for worker $w$, and $V(r_c,s_w(c))$ denotes the utility worker $w$ has for company $c$.

To define the loss in the many-to-one setting, we need to define a non-symmetric notion of alignment of workers and companies.

\begin{defn} [Alignment]
Suppose company $c$ has rank $i$ (as per its public rating). Let $w$ be the worker of rank $d\cdot i$ (also as per its public rating). Then $w$ is aligned with $c$.
Likewise, suppose worker $w'$ has rank $j$.
Let $c'$ be the company with rank $\ceil{j/d}$.
Then $c'$ is aligned with $w'$.
\end{defn}

\begin{defn} [Loss, cont.]
\label{defn::loss-many-to-one} 
Let $c$ be a company and let $w$ be aligned with $c$.
The \emph{loss} $c$ sustains from a match of utility $u$ is defined to be $U(r_w,1) - u$.
Similarly, let $w'$ be a worker and let $c'$ be aligned with $w'$.
The \emph{loss} $w'$ sustains from a match of utility $u$ is defined to be $V(r_{c'},1) - u$.
\end{defn}
